Causal survival embeddings: non-parametric counterfactual inference under censoring

Model-free time-to-event regression under confounding presents challenges due to biases introduced by causal and censoring sampling mechanisms. This phenomenology poses problems for classical non-parametric estimators like Beran's or the k-nearest neighbours algorithm. In this study, we propose a natural framework that leverages the structure of reproducing kernel Hilbert spaces (RKHS) and, specifically, the concept of kernel mean embedding to address these limitations. Our framework has the potential to enable statistical counterfactual modeling, including counterfactual prediction and hypothesis testing, under right-censoring schemes. Through simulations and an application to the SPRINT trial, we demonstrate the practical effectiveness of our method, yielding coherent results when compared to parallel analyses in existing literature. We also provide a theoretical analysis of our estimator through an RKHS-valued empirical process. Our approach offers a novel tool for performing counterfactual survival estimation in observational studies with incomplete information. It can also be complemented by state-of-the-art algorithms based on semi-parametric and parametric models.

==> Abstract.tex <==
\chapter*{Abstract}

Short summary of my thesis.
 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Chapter2.tex <==
\chapter{Assumptions} 



We start with a collection of random variables in the potential outcomes framework \cite{rubin}  $$\{(V^{0}_i,V^{1}_i,Z_i), \quad V \in \{T,C,X\}, \quad i=1,\ldots, n\}$$ such that 

\begin{itemize}
    \item $T^{0}_i,T^{1}_i \in [0, + \infty)$ are potential outcomes of survival times of interest.
    \item $C^{0}_i,C^{1}_i  \in [0, + \infty) $ are potential outcomes of censoring times. 
   
    \item $X^0_i, X^1_i \in \mathbb{R}^p$ are individual vectors of covariates, $p \geq 1$.
     \item $Z_i \in \{0,1\}$ are individual treatment assignment indicators.

\end{itemize}

In practice, when time-to-events are right-censored we instead observe indirectly 
$$\{(T^{*}_i,\Delta_i,Z_i,X_i), \quad i=1,\ldots, n\}$$ where $$T^{*}_i=(1-Z_i)\min\{T^{0}_i,C^0_i\}+Z_i \min\{T^{1}_i,C^1_i\}$$ with $\Delta_i$ the event indicators $$\Delta_i=(1-Z_i)1(T^{0}_i\leq C^0_i)+Z_i 1(T^{1}_i\leq C^1_i)$$and $$X_i=(1-Z_i)X^{0}_i+ Z_i X^{1}_i$$

We denote by $F_U$ the marginal distribution function of each random variable $U$. We use standard notation to denote joint and conditional distributions. For example, $F_{T^0 | Z=1}$ is the distribution of times of the control population given $Z=1$. 


Directed acyclic graph:
\begin{center}
\begin{tikzpicture}[ -Latex,auto,node distance =1 cm and 1 cm,semithick,
    state/.style ={circle, draw, minimum width = 0.7 cm},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}]
    \node[state] (1) {$C$};
    \node[state] (2) [right =of 1] {$\delta$};
    \node[state] (3) [right =of 2] {$T$};
    \node[state] (4) [below right =of 3,xshift=-0.5cm,yshift=-0.0cm] {$X$};
     \node[state] (5) [above right =of 3,xshift=-0.5cm,yshift=-0.0cm] {$Z$};

    \path (1) edge node[above] {} (2);
    \path (3) edge node[above] {} (2);
    \path (4) edge node[above] {} (3);
    \path (5) edge node[above] {} (3);
    \path (5) edge node[above] {} (1);
    \path (4) edge node[above] {} (1);
        \path (4) edge node[above] {} (5);


\end{tikzpicture}
\end{center}



From the directed acyclic graph we read that $$C \indep T $$

ARE WE SURE!!! X IS INFLUENCING BOTH

Note that the existence of an arrow between $C$ and $X$ is not incompatible from the assumption that

$$\delta \indep X | T,Z$$

because it is the \textit{absence} of arrows what permits to conclude conditional independence relations, but not the presence.

For instance, let an underlying model be: 

$$\begin{aligned}
T^0&=f^0(X) +  \varepsilon^0\\
C^0& =f^0(X) +  \omega^0\\
T^1& =f^1(X) +  \varepsilon^1\\
C^1& =f^1(X) +  \omega^1\\
\end{aligned}$$
where $f^0$ and $f^1: \mathcal{X} \longrightarrow \mathbb{R}$ are regular enough maps and $\varepsilon^0,\omega^0,\varepsilon^1,\omega^1$ are normally distributed with mean zero and their respective standard deviations. 
This implies that 


$$\begin{aligned}
\probb (T \leq C | T,Z,X)&=\\&=\probb (T - C\leq 0  | T,X)  \\
&=\probb ((1-Z) (T^0-C^0)+ Z (T^1-C^1) \leq 0 | T,Z,X)\\
&=\probb ((1-Z) (T^0-C^0)+ Z (T^1-C^1)  | T,Z,X) \\
&=\probb ((1-Z) (\varepsilon^0-\omega^0)+ Z (\varepsilon^1-\omega^1)  | T,Z)
\end{aligned}$$

With this, we want to make emphasis that the assumptions are flexible enough to allow for a dependence of $C$ on $X$.

The assumption that the censoring indicator only depends of the covariates through $T$ and the treatment indicator $Z$ is similar to that in \citet*{stute1993,stute1996} where $Z$ still does not appear because this work does not concern the potential outcome framework. 



We depict the assumption of conditional exogeneity stating that the joint distribution satisfies the global Markov property with respect to the following undirected graph:
\begin{center}
\begin{tikzpicture}[auto,node distance =1 cm and 1 cm,semithick,
 every loop/.style={},
    state/.style ={circle, draw, minimum width = 0.7 cm},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}]
 \node[state] (1) {$C^0$};
    \node[state] (2) [right =of 1] {$C^1$};
    \node[state] (3) [right =of 2] {$T^0$};
        \node[state] (4) [right =of 3] {$T^1$};

    \node[state] (5) [below =of 4,xshift=-0.0cm,yshift=-0.0cm] {$X$};
            \node[state] (6) [right =of 5] {$Z$};

 \path (1) edge node[above] {} (2);
    \path (3) edge node[above] {} (4);
        \path (1) edge node[above] {} (5);
                \path (2) edge node[above] {} (5);
        \path (3) edge node[above] {} (5);
            \path (4) edge node[above] {} (5);
            \path (5) edge node[above] {} (6);
\end{tikzpicture}

\end{center}

We limit ourselves to undirected links because it does not make sense to state that the dependence between $T^0$ and $T^1$ goes in one direction or other (same for $C^0$ and $C^1$). Again, this configuration does not prevent $T=(1-Z) T^0+ ZT^1$ from being independent of $C=(1-Z) C^0+ ZC^1$

\section{Derivation of estimator}
Complete with definitions in section 2.3 measure theoretic 
Let the empirical risk be 
$$\hat{R}_ {\lambda}(F):=\frac{1}{n}\sum_{i=1}^nW_i\left\|h_i-F\left(X_i\right)\right\|_{\mathcal{H}}^2+\lambda\|F\|_\mathcal{F}^2$$

Then $$\begin{aligned}
&\hat{R}_ {\lambda}(\hat{F}+G)=\frac{1}{n}\sum_{i=1}^nW_i\left\|h_i-\hat{F}\left(X_i\right) -G\left(X_i\right)\right\|_{\mathcal{H}}^2+\lambda\|\hat{F}+G\|_\mathcal{F}^2= \\
&\frac{1}{n}\sum_{i=1}^nW_i\left(\left\|h_i-\hat{F}\left(X_i\right) \right\|_{\mathcal{H}}^2+\left\|G\left(X_i\right)\right\|_{\mathcal{H}}^2-2\langle h_i-\hat{F}(X_i),{G}(X_i) \rangle_{\mathcal{H}}\right)+\lambda\left(\|\hat{F}\|_\mathcal{F}^2+\|G\|_\mathcal{F}^2 -2 \langle \hat{F},G\rangle_{\mathcal{F}}\right) = \\
&\hat{R}_ {\lambda}(\hat{F}) + \frac{1}{n}\sum_{i=1}^nW_i\left(\left\|G\left(X_i\right)\right\|_{\mathcal{H}}^2-2\langle h_i- \hat{F}(X_i),{G}(X_i) \rangle_{\mathcal{H}}\right)+\lambda\left(\|G\|_\mathcal{F}^2 +2 \langle\hat{F},G\rangle_{\mathcal{F}}\right) = 
\end{aligned}$$ 

Check why but we set

$$ \frac{1}{n}\sum_{i=1}^nW_i\langle h_i- \hat{F}(X_i),{G}(X_i) \rangle_{\mathcal{H}}=\lambda \langle\hat{F},G\rangle_{\mathcal{F}}$$

Use $$\langle\hat{F}, G\rangle_{\mathcal{F}}=\sum_{i=1}^n\langle c_i, G(X_i)\rangle_{\mathcal{H}}$$

So 

$$ \frac{1}{n}\sum_{i=1}^nW_i\langle h_i- \hat{F}(X_i),{G}(X_i) \rangle_{\mathcal{H}}=\lambda \sum_{i=1}^n\langle c_i, G(X_i)\rangle_{\mathcal{H}}$$
Therefore

$$ \sum_{i=1}^n \left(W_i\langle h_i- \hat{F}(X_i),{G}(X_i) \rangle_{\mathcal{H}}-n\lambda \langle c_i, G(X_i)\rangle_{\mathcal{H}}\right)=0$$

Substitute  $$\hat F = \sum_{j=1}^n \Gamma(\cdot ,X_j) c_j$$ and then 

$$\begin{aligned}\langle\hat F(X_i),G(X_ i)\rangle_{\mathcal{H}} & = \langle\hat F,\Gamma(\cdot ,X_i)G(X_ i)\rangle_{\mathcal{F}} = \langle\sum_{j=1}^n \Gamma(\cdot ,X_j) c_j,\Gamma(\cdot ,X_i)G(X_ i)\rangle_{\mathcal{F}}\\& = \sum_{j=1}^n\langle  c_j,\Gamma(X_j ,X_i)G(X_ i)\rangle_{\mathcal{H}} =  \sum_{j=1}^n\langle \Gamma(X_i ,X_j) c_j,G(X_ i)\rangle_{\mathcal{H}}\end{aligned}$$

using the definition of adjoint operator and that $\Gamma^*(X_j ,X_i)=\Gamma(X_i ,X_j)$ 

It is sufficient that for $1 \leq i \leq n$ the following holds 

$$ W_i( h_i- \sum_{j=1}^n \Gamma(X_i ,X_j) c_j)-n\lambda  c_i=0$$

that can be written as 

$$ W_i h_i=\sum_{j=1}^n W_i \Gamma(X_i ,X_j)c_j+n\lambda  c_i\delta_{ij}$$

or in matrix form 

$$W H=(WK+ n\lambda I ) C \Longleftrightarrow  C=(WK + n\lambda I ) ^{-1}WH$$

where $W=\textrm{diag}(W_1, \ldots, W_n)$, $H=(h_1\ldots h_n)^T$, $C=(c_1\ldots c_n)^T$. 

Now the \textbf{conditional} mean embedding evaluated on the covariates of the treated sample $(X^1_1, \ldots,X^1_m )$ is 

$(\hat F(X^1_1) \ldots \hat F(X^1_m))=(\sum_{j=1}^n\Gamma(X^1_1 ,X_j) c_j\ldots\sum_{j=1}^n\Gamma(X^1_m ,X_j) c_j) = C^T\Tilde{K}$

where $\Tilde{K}_{ij}=\Gamma(X_i,X^1_j)$

The \textbf{counterfactual} mean embedding is computed by taking the average of the previous row:

$\hat \mu = C^T\Tilde{K} 1_m $ where $1_m$ is a vector of all ones divided by $m$. 

Summarising

$\hat \mu= ((WK + n\lambda I ) ^{-1}WH)^T\Tilde{K} 1_m = H^T W(KW + n\lambda I ) ^{-1}\Tilde{K} 1_m$

If $H_{ij}=l(T_i,t_j)$, where $t_1,\ldots, t_N$ is a grid of time-points to compute the counterfactual mean embedding, then $\hat \mu$ is a co $N$ rows and 

$\hat \mu^T= 1^T_m \Tilde{K}^T(WK + n\lambda I ) ^{-1}W H  $ is a row with $N$ columns (visually, resembles better to a function of time). 

TODO: explain identification between K and gamma

Remember that K is the matrix and k is the function!!!

\citet*{grune} \citet{pontil} \cite{measure}

% asterisk prints all names, t means opposite as p (parenthesis). 
Modify the prooof with W!!!
\begin{definition}
$$\widehat{\mathcal{C}}^*_{X X} f:=\frac{1}{n} \sum_{i=1}^n W_i k\left(\cdot, X_i\right) f\left({X}_i\right), \quad \widehat{\mathcal{C}}^*_{TX} f=\frac{1}{n} \sum_{i=1}^n W_i\ell\left(\cdot, T^*_i\right) f\left(X_i\right), \quad f \in \textrm{RKHS of } K.$$
\end{definition}
Adapted from \citet*{cme}
\begin{propo}
Let $\hat{\mu}_{\langle 0 \mid 1\rangle}$ be the CME estimator. Then we have
$$
\hat{\mu}_{\langle 0 \mid 1\rangle}=\widehat{\mathcal{C}}^*_{Y X}\left(\widehat{\mathcal{C}}^*_{X X}+\varepsilon I\right)^{-1} \hat{\mu}_{X_1} .
$$

\end{propo}

\begin{proof}
Define $g:=\left(\widehat{\mathcal{C}^*}_{X X}+\varepsilon I\right)^{-1} \hat{\mu}_{X_1}$. \\ Since $\hat{\mu}_{X_1}=\left(\widehat{\mathcal{C}^*}_{X X}+\varepsilon I\right) g=\frac{1}{n} \sum_{j=1}^n W_j k\left(\cdot, X_j\right) g\left(X_j\right)+\varepsilon g$, \\ we have $\hat{\mu}_{X_1}\left(X_l\right)=\frac{1}{n} \sum_{j=1}^n W_j k\left(X_{l}, X_j\right) g\left(X_j\right)+\varepsilon g\left(X_{l}\right)=\frac{1}{n}(KW\boldsymbol{g})_{l}+\varepsilon \boldsymbol{g}_{l}$ for all $l=1, \ldots, n$, where $K \in \mathbb{R}^{n \times n}$ with $K_{i j}=k\left(X_i, X_j\right)$ and $\boldsymbol{g}=\left(g\left(X_1\right), \ldots, g\left(X_n\right)\right)^{\top} \in \mathbb{R}^n$. Therefore $\boldsymbol{\mu}=$ $\frac{1}{n}(KW+n \varepsilon I) \boldsymbol{g}$, where $\boldsymbol{\mu}:=\left(\hat{\mu}_{X_1}\left(X_1\right), \ldots, \hat{\mu}_{X_1}\left(X_n\right)\right)^{\top}=\widetilde{K} 1_m$, where $1_m=(1 / m, \ldots, 1 / m)^{\top}$ and $\widetilde{K} \in \mathbb{R}^{n \times m}$ with $\widetilde{K}_{i j}=k\left(X_i, X_j^{1}\right)$. Thus $\boldsymbol{g}=n(K+n \varepsilon I)^{-1} \boldsymbol{\mu}$. Lastly, we use the definition of $\widehat{\mathcal{C}^*}_{Y X}$ to express $\hat{\mu}_{\langle 0 \mid 1\rangle}=\frac{1}{n} \sum_{i=1}^n W_i\ell\left(\cdot, Y_i\right) g\left(X_i\right)=\sum_{i=1}^n W_i\beta_i \ell\left(\cdot, Y_i\right)$, where $\beta=\left(\beta_1, \ldots, \beta_n\right)^{\top}=$ $n^{-1} \boldsymbol{g}=(KW+n \varepsilon I)^{-1} \boldsymbol{\mu}$, which is the original expression of the counterfactual mean embedding estimator $\hat{\mu}_{\langle 0 \mid 1\rangle}$.
\end{proof}


\begin{enumerate}
\item $\sup _{X \in \mathcal{X}} k(X, X)<\infty$ and $\sup _{T \in \mathcal{Y}} \ell(T, T)<\infty$

\item The distribution $\mathbb{P}_{X_1}$ is absolutely continuous with respect to $\mathbb{P}_{X_0}$ with the Radon-Nikodym derivative $g:=\mathrm{d}_{X_1} / \mathrm{d} \mathbb{P}_{X_0}$ satisfying $g \in L_2\left(\mathbb{P}_{X_0}\right)$.
\item $g$ satisfies $g \in \operatorname{Range}\left(T^\alpha\right)$ for a constant $\alpha \geq 0$. Then for any $\varepsilon_n>0$ such that $\varepsilon_n \rightarrow 0$ as $n \rightarrow \infty$, we have
\item $\left(X_1, T_1^{*}\right), \ldots,\left(X_n, T_n^{*}\right)$ are i.i.d. observations of the random variables $\left(X^0, T^{0*}\right)$, and $X_1^1 \ldots, X_m^1 $ are i.i.d. observations of the random variable $X^1$, with $n=m$.


\end{enumerate}
Proof of Theorem 11 in \citet*{fukumizubayes}: \begin{equation*}
\begin{split}
& \left\|\widehat{\mathcal{C}^*}_{T X}\left(\widehat{\mathcal{C}^*}_{X X}+\varepsilon_n I\right)^{-1} \widehat{\mu}_{X_1}-\mathcal{C}_{T X}\left( \mathcal{C}_{X X}+\varepsilon_n I\right)^{-1} \mu_{X_1} \right\|_{\mathcal{F}} \leq \\ \leq &\left\|\widehat{\mathcal{C}^*}_{T X}\left(\widehat{\mathcal{C}}_{X X}+\varepsilon_n I\right)^{-1}\left(\widehat{\mu}_{X_1}-\mu_{X_1}\right)\right\|_{\mathcal{F}} \\ 
+ &\left\|\left(\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\right)\left(\mathcal{C}_{X X}+\varepsilon_n I\right)^{-1} \mu_{X_1}\right\|_{\mathcal{F}} \\
+ & \left\|\widehat{\mathcal{C}^*}_{TX}\left(\widehat{\mathcal{C}^*}_{X X}+\varepsilon_n I\right)^{-1}\left(\mathcal{C}_{XX}-\widehat{\mathcal{C}^*}_{X X}\right)\left(\mathcal{C}_{X X}+\varepsilon_n I\right)^{-1} \mu_{X_1}\right\|_{\mathcal{F}}
\end{split}
\end{equation*}

Second term (use Lemma 24 in \citet{cme} and assumptions i, ii and iii)
\begin{align*}
\left\|\left(\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\right)\left(\mathcal{C}_{X X}+\varepsilon_n I\right)^{-1} \mu_{X_1}\right\|_{\mathcal{F}} & \leq\left\|\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\right\|\left\|\left(\mathcal{C}_{X X}+\varepsilon_n I\right)^{-1} \mu_{X_1}\right\|_{\mathcal{H}} \\
& \leq\left\|\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\right\| c_\alpha \varepsilon_n^{\min (-1 / 2+\alpha, 0)}   \\
& =O_p\left(n^{-1 / 2} \varepsilon_n^{\min (-1 / 2+\alpha, 0)}\right) 
\end{align*}

Provided that we show the tight uniform bound $\left\|\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\right\|=O_p\left(n^{-1 / 2}\right)$

\begin{definition}[\cite{reed1980methods}]
 Let $\mathcal{H}$ be a separable infinite-dimensional Hilbert space with complete orthonormal basis $\left(e_i\right)_{i \in \mathbb{N}}$. Suppose $\mathcal{C}: \mathcal{H} \rightarrow \mathcal{H}$ is a bounded linear map with the property that
$$
\|\mathcal{C}\|_{H S}^2:=\sum_{i=1}^{\infty}\left\|\mathcal{C} e_i\right\|_\mathcal{H}^2<\infty .
$$
Operators $\mathcal{C}$ with this property are called Hilbert-Schmidt operators, and $\|\mathcal{C}\|_{H S}$ is their so-called Hilbert-Schmidt norm.
\end{definition}
\begin{lemma}

$$\|\mathcal{C}\| \leq \|\mathcal{C}\|_{H S}$$

\end{lemma}

\begin{lemma}

$$\|\widehat{\mathcal{C}^*}_{T X}-\mathcal{C}_{T X}\|_{H S}^2= \left\|\frac{1}{n} \sum_{i=1}^nW_i\left(K_i-\frac{1}{n} \sum_{j=1}^nW_j F_j\right)\left(L_i-\frac{1}{n} \sum_{j=1}^n W_jG_j\right)-E[F G]\right\|_{\mathcal{H}\otimes\mathcal{F}}^2$$

\end{lemma}


\begin{proof}
See \cite{fukumizu07a}
\end{proof}


\begin{align*}
&\left\|\frac{1}{n} \left(\sum_{i=1}^nW_iK_iL_i-\frac{2}{n} \left(\sum_{i=1}^nW_i K_i\right)\left(\sum_{i=1}^nW_iL_i\right) + \frac{1}{n^2}\left(\sum_{i=1}^nW_i K_i\right)\left(\sum_{i=1}^nW_iL_i\right)\left(\sum_{i=1}^nW_i\right)\right)-E[F G]\right\|_{\mathcal{H}\otimes\mathcal{F}}\\
&\left\|\frac{1}{n} \sum_{i=1}^nW_iK_iL_i-2 \left(\frac{1}{n}\sum_{i=1}^nW_i K_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_iL_i\right) + \left(\frac{1}{n}\sum_{i=1}^nW_i K_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_iL_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_i\right)-E[F G]\right\|_{\mathcal{H}\otimes\mathcal{F}} \\
&\left\|\frac{1}{n} \sum_{i=1}^nW_iK_iL_i-E[F G]-\left(2 -\frac{1}{n}\sum_{i=1}^nW_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_i K_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_iL_i\right) \right\|_{\mathcal{H}\otimes\mathcal{F}} \\
&\leq \left\|\frac{1}{n} \sum_{i=1}^nW_iK_iL_i-E[F G]\right\|_{\mathcal{H}\otimes\mathcal{F}} +\left|2 -\frac{1}{n}\sum_{i=1}^nW_i\right|\left\|\left(\frac{1}{n}\sum_{i=1}^nW_i K_i\right)\left(\frac{1}{n}\sum_{i=1}^nW_iL_i\right) \right\|_{\mathcal{H}\otimes\mathcal{F}}
\\
&\leq \left\|\frac{1}{n} \sum_{i=1}^nW_iK_iL_i-E[F G]\right\|_{\mathcal{H}\otimes\mathcal{F}} +\left|2 -\frac{1}{n}\sum_{i=1}^nW_i\right|\left\|\left(\frac{1}{n}\sum_{i=1}^nW_i K_i\right)\right\|_{\mathcal{H}}\left\|\left(\frac{1}{n}\sum_{i=1}^nW_iL_i\right) \right\|_{\mathcal{F}} 
\end{align*}

explain why norm factorises into norm of marginal rkhs

\begin{definition}[Hadamard-differentiability, \cite{van2000asymptotic}]
Let $\mathbb{D}$ and $\mathbb{E}$ be normed spaces. A map $\phi: \mathbb{D}_\phi \subset \mathbb{D} \mapsto \mathbb{E}$ is Hadamard-differentiable at $\theta \in \mathbb{D}$, tangentially to a set $\mathbb{D}_0 \subset \mathbb{D}$, if there exists a continuous linear map $\phi_\theta^{\prime}: \mathbb{D} \mapsto \mathbb{E}$ such that
$$
\frac{\phi\left(\theta+t_n h_n\right)-\phi(\theta)}{t_n} \rightarrow \phi_\theta^{\prime}(h),
$$
as $n \rightarrow \infty$, for all converging sequences $t_n \rightarrow 0$ and $h_n \rightarrow h \in \mathbb{D}_0$, with $h_n \in \mathbb{D}$ and $\theta+t_n h_n \in \mathbb{D}_\phi$ for all $n \geq 1$ sufficiently large.
\end{definition}
\begin{definition}
For any interval $A \subset \mathbb{R}$, $D A$ is the space of cadlag (right-continuous with left-hand limits) real functions on $A$ with the uniform norm.
\end{definition}

\begin{lemma}
Let $\mathbb{D}=D[0,1]$ and $\mathbb{D}_\phi=\{f \in D[0,1]:|f|>0\}$. Then the function $\phi: \mathbb{D}_\phi \mapsto \mathbb{E}=D[0,1]$ defined by $\phi(g)=1 / g$ is Hadamard-differentiable for any $\theta \in \mathbb{D}_\phi$.  
\end{lemma}

\begin{proof}

$$
\frac{\phi\left(\theta+t_n h_n\right)-\phi(\theta)}{t_n}=\frac{1}{t_n\left(\theta+t_n h_n\right)}-\frac{1}{t_n \theta}=-\frac{h_n}{\theta\left(\theta+t_n h_n\right)} \rightarrow-\frac{h}{\theta^2},
$$

for any converging sequences $t_n \downarrow 0$ and $h_n \rightarrow h \in \mathbb{D}$, with $h_n \in \mathbb{D}$ and $\theta+t_n h_n \in \mathbb{D}_\phi$ for all $n \geq 1$.
\end{proof}
\cite{kosorok2008introduction}



\begin{align*}\frac{1}{n}\sum_{i=1}^nW_iK_i&=\frac{1}{n}\sum_{i=1}^nW_i(k(,X_i)-\mu_0)=\frac{1}{n}\sum_{i=1}^n(W_ik(,X_i)-W_i\mu_0)\\&=\frac{1}{n}\sum_{i=1}^nW_ik(,X_i)-\mu_0+\mu_0-\mu_0\left(\frac{1}{n}\sum_{i=1}^nW_i\right)=\\
&=\left(\frac{1}{n}\sum_{i=1}^nW_ik(,X_i)-\mu_0\right)+\mu_0\left(1-\frac{1}{n}\sum_{i=1}^nW_i\right)=\\
\end{align*}

\begin{align*}
\frac{1}{n}\sum_{i=1}^nW_ik(,X_i)-\mu_0=\int _\mathcal{X}k(\cdot,X)\frac{d\hat{F}^1}{\hat{G}} -\int _\mathcal{X}k(\cdot,X)\frac{dF^1}{G}=\nu(\hat{F}^1,\hat{G})- \nu({F}^1,{G})
\end{align*}


Let, tor $n \geq 1$,
$$
S_n=\sum_{i=1}^n \Delta_i k\left(\cdot, X_i\right)
$$
and
$$
\Lambda_n=\sqrt{n}\left(\frac{S_n}{n}-\mathcal{I}_\mu\right) .
$$
First of all, as
$$
\int k\left(\cdot, X\right) d F^1=E\left(k\left(\cdot, X\right)\right)
$$
we have, by the strong law of large numbers, almost sure convergence of $S_n / n$ towards $\mathcal{I}_\mu$ as $n$ tends to infinity. Second it is possible to prove by using the Hilbert space version of the Central Limit Theorem in \citet*{ledoux1991probability} that the sequence $\left(\Lambda_n\right)_{n \geq 1}$ converges weakly to a centered gaussian process \citep*{berlinet2011reproducing}

Now adapt page 242 kosorok or assume it is true to proof that integration is had diff

taking B=kF1 and A = 1/G
% https://metaphor.ethz.ch/x/2022/hs/401-3461-00L/sc/Exercises/Exercises_6/FAI2022_Solutions_6.pdf

From \cite{Muandet_2017} 


\cite{fukumizu07a} bound term by term (better use muandet isomorphism)
\cite{Muandet_2017} review 
\cite{fukumizu2009kernel} empirical process 

https://math.stackexchange.com/questions/142614/operator-norm-and-hilbert-schmidt

add comments to assumptions in page 21




\section{To include a picture}
\begin{figure}[hbt!]%--- Picture 'H'ere, 'B'ottom or 'T'op; '!' Try to
                    %impose your will to LaTeX
  \epsfCfile{.85}{geys-2kern} %<< no file extension
  %%         --- .85 stands for 85% of text width
  \caption[Geyser data: binned histogram, Silverman's and another
  kernel]%<<-- Legend for the list of figures at the beginning of you thesis
  {Old Faithful Geyser eruption lengths, $n=272$; binned data and two
    (Gaussian) kernel density estimates ($\times 10$) with $h=h^*= .3348$
    and $h= .1$ (dotted).}% legend displayed below the graph.
  \label{fig:geys1}
\end{figure}

Or also with \texttt{includegraphics}:
\begin{figure}[hbt!]%--- Picture 'H'ere, 'B'ottom or 'T'op; '!' Try to
                    %impose your will to LaTeX
  \centering
  \includegraphics[width=.5\textwidth]{geys-2kern} %<< no file extension
  %%         --- .5\textwidth stands for 50% of text width
  \caption[Geyser data: binned histogram, Silverman's and another
  kernel]%<<-- Legend for the list of figures at the beginning of you thesis
  {Old Faithful Geyser eruption lengths, $n=272$; binned data and two
    (Gaussian) kernel density estimates ($\times 10$) with $h=h^*= .3348$
    and $h= .1$ (dotted).}% legend displayed below the graph.
  \label{fig:geys2}
\end{figure}

\section{To make a proof}
\begin{proof}
  $1 + 1 = 2$
\end{proof}

\section{To include \Rp code}
See information in Appendix~\ref{app:complement}.


\section{Other information}
Put a text between quotes: make sure to use nice quotes, such as ``quote''.

Cite an article or book you refer shortly here, and then listed in the bibliography: \cite{ReferenceKey}. 
%%--> in file   myReferences.bib  (same directory)
Or mention that \citeauthor{HamF85} (a person) or \citeauthor{StaWW91} (two
persons) have already done quite a bit work.

Referencing a different part of your work: please refer to Appendix \ref{app:complement}.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Epilogue.tex <==
\chapter*{Epilogue}
\label{s:Epilogue}

A few final words.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Introduction.tex <==
\chapter{Introduction} 

Description of the work. Prepare the reader for the following chapters.

You will cite literature here, typically, but

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Notation.tex <==
\section*{Notation}
\label{c:Notation}


$\mathcal{X}$ covariate space \\
$\mathcal{T}$ target space \\
$l$ kernel defined on the target space \\
$k$ kernel defined on the covariate space \\
$\mathcal{G}$ RKHS of $k$ \\ % should be H
$\mathcal{H}$ RKHS of $l$ \\ % should be F \\
$\mathcal{F}$ $\mathcal{H}$-valued RKHS on $\mathcal{X}$ % should be G


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Preface.tex <==
\chapter*{Preface}

First words and acknowledgements.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 


==> Summary.tex <==
\chapter{Summary}
\label{s:Summary}

Summarize the presented work. Why is it useful to the research field or institute?


\section{Future Work}
\label{ss:FutureWork}

Possible ways to extend the work.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MasterThesisSfS"
%%% End: 

